PDA: Semantically Secure Time-Series Data Analytics with Dynamic Subgroups

Third-party analysis on private records is becoming increasingly important due to the widespread data collection for various analysis purposes. However, the data in its original form often contains sensitive information about individuals, and its publication will severely breach their privacy. In this paper, we present a novel Privacy-preserving Data Analytics framework PDA, which allows a third-party aggregator to obliviously conduct many different types of polynomial-based analysis on private data records provided by a dynamic sub-group of users. Notably, every user needs to keep only O(n) keys to join data analysis among O(2^n) different groups of users, and any data analysis that is represented by polynomials is supported by our framework. Besides, a real implementation shows the performance of our framework is comparable to the peer works who present ad-hoc solutions for specific data analysis applications. Despite such nice properties of PDA, it is provably secure against a very powerful attacker (chosen-plaintext attack) even in the Dolev-Yao network model where all communication channels are insecure.

==> conclusion_v1.tex <==
\section{Conclusion}\label{section:conclusion}

In this paper, we successfully designed a privacy-preserving data aggregation scheme which relies on  our novel arithmetic protocol. Our arithmetic protocol, which allows a group of participants to compute their sum or product privately, fulfils all the aforementioned requirements for data aggregations in a real life, and is also provably secure against $n_{min}-2$ cooperative attackers. Notably, our scheme supports infinitely many formats of data aggregation among any group of participants with only $\theta(n)$ keys while other similar works require $\theta(2^n)$ keys or more.

However, our scheme does disclose single product terms in the polynomial, which gives unnecessary information to the attackers. To prevent such leakage is one of the important future directions.

==> design_v1.tex <==
\section{Our Construction}\label{section:design}

%We first show how to achieve arithmetic (sum \& product calculation) in a privacy-preserving manner while satisfying aforementioned requirements. This arithmetic protocol will be used to implement data aggregation scheme under two models in the next section.

%\subsection{Building Block}
%
%In \cite{jung2013privacypreserving}, we designed a privacy-preserving multivariate polynomial evaluation (MPEP hereafter). We proposed a random sharing technique such that independently generated random keys $R_1,\cdots,R_n$ satisfy $\prod_{i=1}^{n}R_i=1~(\text{mod } p)$ where $p$ is a large number. Then, each party reports $R_i\cdot m_i$ instead of $m_i$, and the product $\prod m_i$ can be achieved from $\prod R_im_i$ without disclosing individual $m_i$. This is used to implement the privacy-preserving sum calculation, which we also show in our construction.


%Secondly, in order to implement the privacy-preserving sum calculation, they used the following \textit{binomial property} to calculate a sum via a product:
%
%{\footnotesize\vspace{-14pt}
%\begin{displaymath}
%\begin{split}
%\prod{(1+s)^{x_i}}&=(1+s)^{\sum x_i} = \sum_{i=0}^{\sum x_i}{\binom{\sum x_i}{i} s^i} \\
%&= 1+s\sum{x_i} \mod s^2
%\end{split}
%\end{displaymath}\vspace{-8pt}}
%
%By exploiting this property, sum is indirectly computed by the product, and the above privacy-preserving product calculation can be used. 

%We will use this as a building block to design a flexible scheme, which supports data aggregation among any combination of participants. 
%One na\"{i}ve idea to achieve the flexibility is to let all non-participating users in the system to provide a null value (0 in the sum and 1 in the product calculation) as their inputs, but this requires all users to be online every time an aggregation is conducted, and it also incurs unnecessary computation and communication overhead for the null values.

%\subsubsection{Paillier Cryptosystem}
%Paillier Cryptosystem is a famous homomorphic encryption (\cite{paillier1999public}), which is shown below. It is an additive homomorphic cryptosystem, i.e., given the public keys and the ciphertext of $m_1$ and $m_2$, anyone can compute the ciphertext of $m_1+m_2$.
%
%{\footnotesize\vspace{-2pt}
%\begin{table}[h]
%\centering
%\begin{tabular}{|l|}
%\hline
%~~~~~~~~~~~~~~~~~~~~~~\textbf{Paillier Cryptosystem}\\
%\textbf{System parameter}: two same-length prime numbers $p,q$\\
%\textbf{Public key}: modulus $n=pq$\\
%\textbf{Private key}: $\lambda=(p-1)(q-1),\mu=\lambda^{-1}$ mod $n$\\
%\textbf{Encryption}: $c=E(m,r)=g^{m}r^n~\mod n^2$\\ ~~~~~~~~~~~~~~~~where $r\in \mathbb{Z}^*_{n}$ is a random number.\\
%\textbf{Decryption}: $m=D(c)=L(c^\lambda\mod n^2)\cdot \mu~\mod n$\\
%~~~~~~~~~~~~~~~~where $L(x)=\frac{x-1}{n}~\mod n$\\
%\textbf{Self-blinding}: $E(m,r)\cdot \hat{r}^n=E(m,r\hat{r})$\\\hline
%\end{tabular}
%\end{table}\vspace{-8pt}}




%\subsection{Grouping Approach with $\theta(n^{5})$ Keys}
%
%
%Since MPEP is able to privately evaluation a multivariate polynomial, we can use the following grouping technique to achieve any-combination data aggregation among $n$ participants $\{1,\cdots,n\}$. For simplicity, we only describe how to achieve the product $\prod_{i\in \mathcal{P}} x_i$ among chosen subset $\mathcal{P}$ of participants, but this can be generalized to a polynomial evaluation as in \cite{jung2013privacypreserving}.
%
%For any combination of 3-out-of-$n$ participants, we use the random sharing technique in \cite{jung2013privacypreserving} to generate three secret keys $\{R^{(3)}_i\}_{i=x,y,z}$ whose product is 1 ($\text{mod}~ p$) for any $x,y,z$. This leads to $\binom{n}{3}$ secret numbers for each participant. We also generate four secret keys $\{R^{(4)}_i\}~s.t.~\prod R^{(4)}_i=1$  for any 4-participant combinations ($\binom{n}{4}$ keys for each participant) and five secret keys $\{R^{(5)}_i\}~s.t.~\prod R^{(5)}_i=1$  for any 5-participant combinations ($\binom{n}{5}$ keys for each participant) likewise.
%
%Then, when a subset of participants $\mathcal{P}\subseteq\{1,\cdots,n\}$ need to compute a product of their private data, the $\mathcal{P}$ is grouped into $k+1$ groups as follows ($k=0,1,\cdots$), where $|\mathcal{P}|$ refers to the size of the group:
%
%{\footnotesize\vspace{-6pt}
%\begin{displaymath}
%\mathcal{P}\rightarrow \begin{cases} \text{$k+1$ 3-participants groups} & \text{$|\mathcal{P}|=3k+3$} \\ 
%\text{$k$ 3-participants groups \& one 4-participants group} & \text{$|\mathcal{P}|=3k+4$} \\
%\text{$k$ 3-participants groups \& one 5-participants group} &\text{$|\mathcal{P}|=3k+5$} 
%\end{cases}
%\end{displaymath}\vspace{-6pt}}
%
%The 3-participant groups, 4-participant group, 5-participant group use their secret keys $R^{(3)}_i,R^{(4)}_i,R^{(5)}_i$ respectively to report their private data, and each individual privacy is preserved. We cannot have 2-participants group since at least 3 participants should take part in the protocol to preserve privacy.
%
%Obviously, this approach requires every participant to hold $\theta(\binom{n}{5})=\theta(n^5)$ keys to let $\theta(2^n)$ subsets of $n$ participants to privately calculate the product. Although this reduced the key complexity from an exponential growth to a polynomial growth, $n^5$ is still too high in resource-bounded platforms. More importantly, this reveals intermediate product result among 3-participants group, 4-participant group or 5-participant group, which is of great usage to adversaries.

\subsection{Our Novel Approach with $\theta(n)$ Keys}

For simplicity, we describe our novel idea on how to achieve the sum among any group of participants $\mathcal{P}$ ($|\mathcal{P}|=k$), and generalize it to a polynomial evaluation later.

For a special polynomial $poly^{(k-1)}(x)=\sum_{j=1}^{k-1}a_jx^j$ whose constant term is 0, we have $poly^{(k-1)}(0)=0$. Then, if we are able keep $poly^{(k-1)}(i)$ secret to any participant $j\neq i$, each participant $i\in \mathcal{P}$ owns a secret number $poly^{(k-1)}(i)\mathcal{L}_{i,\mathcal{P}}(0)$. Since sum of any $k$ participants' $poly^{(k-1)}(i)\mathcal{L}_{i,\mathcal{P}}(0)$ is always 0, the secret numbers can be used to mask participants' private data when computing the sum. That is, each participant $i$ sends out $x_i+poly^{(k-1)}(i)\mathcal{L}_{i,\mathcal{P}}(0)$ instead of $x_i$ to keep his data secret. To compute a sum among a different set $\mathcal{P}'$ of $k$ participants, participant $i$ only needs to change the Lagrange coefficient accordingly, which is a trivial job.

% $i$ can send out $R_i^{(k)}+x_i$ instead of $x_i$ when computing $\sum_{i=1}^k x_i$ to mask his raw data. 

In order to allow any subset of $n$ participants to compute their sum, each participant $i$ needs to privately compute and hold $poly^{(k-1)}(i)$ for all $k=3,\cdots,n$, and whenever there are $k$ participants $\mathcal{P}$ joining the sum calculation, participant $i$ can use $poly^{(k-1)}(i)\mathcal{L}_{i,\mathcal{P}}(0)$ to mask his original data. Obviously, this approach only requires $\theta(n)$ keys to store, which is a great improvement compared with $\theta(2^n)$ or $\theta(n^5)$.

We use the privacy preserving sum protocol proposed in \cite{jung2013privacypreserving} to privately compute all $R_i^{(k)}$'s without anyone knowing other's secret number, and further extend the sum calculation to the general polynomial evaluation. Details are shown in the following construction.




\subsection{Arithmetic Protocol Construction}

\noindent \textsc{Setup($1^\kappa$)} $\rightarrow$ $\PK$

Setup algorithm takes $\kappa$ as the security parameter and chooses a large prime number $p$ of length $\kappa$, i.e., $p\in 1||\{0,1\}^{\kappa-1}$. It picks a random number $g\in\zgroup_p$, and the public key is published as $\PK(p,g)$.\medskip


\noindent \textsc{Initialize}($\PK$) $\rightarrow$ $\{\MK_i\}_{i=1,\cdots,n}$

This algorithm uses the random sharing technique proposed in \cite{jung2013privacypreserving} to let each participant $i$ independently and individually compute a secret number $\mathcal{R}_i\in\zgroup_{p^2(p-1)^2}$ such that the overall product $\prod_{i=1}^n\mathcal{R}_i=1\mod p^2(p-1)^2$. Then, participant $i$'s master key is $\MK_i=\mathcal{R}_i$, which will be used to mask the secret values for key generation.

We direct the readers to \cite{jung2013privacypreserving} for technical details of the random sharing. The only difference in this paper is that the algorithm should pick a random number $g_1\in\zgroup_{p^2(p-1)^2}$ such that $\gcd(g_1,p^2(p-1)^2)=1$.\bigskip

\noindent \textsc{Keygen($\PK$)} $\rightarrow$ $\{\SK_i\}_{i=1,\cdots,n}$

Firstly, every participant $i$ individually and randomly picks $k-1$ numbers $\{r_{i,j}^{(k)}\in \zgroup_{p(p-1)}\}_{j=1,\cdots,k-1}$ for all $k=n_{min},\cdots,n$. Then, every participant $i$ holds $k-n_{min}$ sets of random numbers\vspace{-8pt}

\begin{displaymath}\begin{split}
&\{r_{i,1}^{(n_{min})},r_{i,1}^{(n_{min}+1)},\cdots,r_{i,1}^{(n)}\},\\
&\{r_{i,2}^{(n_{min})},r_{i,2}^{(n_{min}+1)},\cdots,r_{i,2}^{(n)}\},\\
&\cdots,\\
&\{r_{i,k-1}^{(n_{min})},r_{i,k-1}^{(n_{min}+1)},\cdots,r_{i,k-1}^{(n)}\}
\end{split}\end{displaymath}


\noindent which are kept secret to anyone else. Then, the sub-algorithm \textsf{$Keygen_i(\PK,\MK_i)\rightarrow\SK_i$} is executed for all participant $i\in\{1,\cdots,n\}$.





\floatname{algorithm}{Sub-Algorithm}
\begin{algorithm}
\caption{$Keygen_i$}
\textbf{Input}: $\PK,\MK_i$\\
The following process is repeated for all $k=n_{min},\cdots,n$.


\begin{algorithmic}[1]

\STATE Every participant $j$ locally computes his secret polynomial-share as:\vspace{-8pt}

%{\footnotesize\vspace{-8pt}
\begin{displaymath}
poly_{j}^{(k-1)}(i)=ir_{j,1}^{(k)}+\cdots +i^{k-1}r_{j,k-1}^{(k)}~~(\text{mod}~p(p-1))
\end{displaymath}
%\vspace{-8pt}}

\STATE Every participant $j$ computes\vspace{-8pt}

%{\footnotesize\vspace{-3pt}
\begin{displaymath}
c_{j,i}^{(k)}=\MK_j (1+p(p-1))^{poly_j^{(k-1)}(i)}~~(\text{mod}~p^2(p-1)^2)
\end{displaymath}
%\vspace{-14pt}}

\STATE Every participant $j$ except $i$ sends $c_{j,i}^{k}$ to the participant $i$.

\STATE Participant $i$ computes the following product:\vspace{-8pt}

%{\footnotesize\vspace{-8pt}
\begin{displaymath}\begin{split}
x_i^{(k)}&=\prod_{j=1}^{n}c_{j,i}^{(k)}=\prod_{j=1}^{n}\MK_i (1+p(p-1))^{\sum_{j=1}^npoly_{j}^{(k-1)}(i)}\\&=(1+p(p-1))^{\sum_{j=1}^npoly_{j}^{(k-1)}(i)}~~\text{(mod } p^2(p-1)^2)
\end{split}\end{displaymath}
%\vspace{-6pt}}

\noindent Then, he computes \vspace{-8pt}

%{\footnotesize\vspace{-12pt}
\begin{displaymath}\begin{split}
&poly^{(k-1)}(i)\\
=&\frac{x_i^{(k)}-1~~~\text{(mod }p^2(p-1)^2\text{)}}{p(p-1)}~~~\text{(mod }p(p-1))\\
=&\sum_{j=1}^npoly_j^{(k-1)}(i)~~(\text{mod}~p(p-1))\\
=&i\sum_{j=1}^nr_{j,1}^{(k)}+\cdots +i^{k-1}\sum_{j=1}^nr_{j,k-1}^{(k)}~~(\text{mod}~p(p-1))
\end{split}\end{displaymath}
%\vspace{-8pt}}

\STATE Participant $i$ sets his secret key $R_{i}^{(k)}:=poly^{(k-1)}(i)$.

\end{algorithmic}

\textbf{Output}: $\SK_i(R_i^{(n_{min})},\cdots,R_i^{(n)})$
\end{algorithm}
Essentially, the $Keygen_i$ let every participant uses his random numbers to generate the partial polynomial $poly_j^{(k-1)}(i)$, and all participants engage in the privacy-preserving sum calculation (described in the $Keygen_i$) to let participant $i$ secretly achieves $poly^{(k-1)}(x)$. Then, only the participant $i$ knows the point $(i,poly^{(k-1)}(i))$ of the polynomial $poly^{(k-1)}(x)$ (modulo omitted), but the polynomial is unknown to anyone due to the independently picked random numbers. Furthermore, everyone's polynomial-share is masked by his secret master key $\mathcal{R}_j$, therefore it is hard to recover each polynomial-share to recover the polynomial.\bigskip


\noindent \textsc{Encrypt($\PK,\SK_i,\mathcal{P},x_i$)} $\rightarrow$ $\mathcal{E}^+(x_i)$ or $\mathcal{E}^{\times}(x_i)$

Given a set of participants $\mathcal{P}$ who need to jointly compute the sum $\sum_{i\in \mathcal{P}}x_i$ or the product $\prod_{i\in\mathcal{P}}x_i$, the encryption algorithm computes $i$'s Lagrange coefficient $\mathcal{L}_{i,\mathcal{P}}(0)$ and encrypts the private data $x_i$ as follows, where $\mathcal{E}^+$ and $\mathcal{E}^{\times}$ refers to the additive ciphertext for the sum calculation and the multiplicative ciphertext for the product calculation respectively.

{\vspace{-6pt}
\begin{displaymath}\begin{split}
\mathcal{E}^+(x_i)&=x_i+R_i^{(|\mathcal{P}|)}\cdot \mathcal{L}_{i,\mathcal{P}}(0)~~(\text{mod}~p)\\
\mathcal{E}^{\times}(x_i)&=x_i\cdot g^{ R_i^{(\abs*{\mathcal{P}})}\cdot \mathcal{L}_{i,\mathcal{P}}(0)}~~(\text{mod}~p)
\end{split}\end{displaymath}\vspace{-2pt}}

\noindent \textsc{Decrypt}($\PK,\{\mathcal{E}^*(x_i)\}_{i\in \mathcal{P}}$) $\rightarrow$ $\sum_{i\in\mathcal{P}}x_i$ or $\prod_{i\in\mathcal{P}}x_i$

Given the set of ciphertexts $\{\mathcal{E}^*(x_i)\}_{i\in \mathcal{P}}$, the decryption algorithm computes $\sum_{i\in\mathcal{P}}\mathcal{E}^+(x_i)$ (mod $p$) if ``$*$'' is ``$+$'', or computes $\prod_{i\in\mathcal{P}}\mathcal{E}^{\times}(x_i)$ (mod $p$) otherwise. The result is sum of $x_i$'s or product of $x_i$'s respectively (modulo $p$).



\subsection{Correctness}

Any component $R_{i}^{(k)}$ in the encryption key $\SK_i$ is the value of the polynomial $poly^{(k-1)}(i)\mod p(p-1)$. Then, according to the polynomial interpolation (Section \ref{section:preliminary}), we have the following for a set of $k$ participants $\mathcal{P}$:

{\vspace{-4pt}
\begin{displaymath}\begin{split}
&\Sigma_0=\sum_{i\in\mathcal{P}}R_{i}^{(k)}\mathcal{L}_{i,\mathcal{P}}(0)=poly^{(k-1)}(0)=0\mod p(p-1)\\
&\rightarrow 
\begin{cases}
\Sigma_0=0\mod p \\
\Sigma_0=0\mod (p-1)\rightarrow g^{\Sigma_0}=1\mod p
\end{cases}
\end{split}\end{displaymath}\vspace{-4pt}
}

\noindent The last implication is true because $p$ is a prime number and thus $\phi(p)=p-1$. Then, we have:

{\footnotesize
\begin{displaymath}
\begin{cases}
\sum_{i\in\mathcal{P}}\mathcal{E}^+(x_i)=\sum_{i\in\mathcal{P}}(x_i+R_{i}^{(k)}\mathcal{L}_{i,P}(0))=\sum_{i\in\mathcal{P}}x_i\mod p \\
\prod_{i\in\mathcal{P}}\mathcal{E}^{\times}(x_i)=\prod_{i\in\mathcal{P}}x_ig^{R_{i}^{(k)}\mathcal{L}_{i,P}(0)}=\prod_{i\in\mathcal{P}}x_i\mod p
\end{cases}
\end{displaymath}
}

\noindent which concludes the correctness of the sum and product calculation.

==> evaluation_v1.tex <==
\section{Performance Evaluation}\label{section:performance}


\subsection{Storage Complexity}
We require every participant to store one master key $\MK_i$ and a set of $n-n_{min}$ encryption keys $\{R_i^{(k)}\}_{k=n_{min},\cdots,n}$. Lagrange coefficient $\mathcal{L}_{i,\mathcal{P}}(0)$ needed in encryption can be computed according to the group of participants $\mathcal{P}$ and their public IDs when needed. Therefore, the storage complexity is $\theta(n)$, where $n$ is the known upper bound of the number of participants.

\subsection{Communication Overhead}

The communication overhead in terms of transmitted bits is summarized in the Table \ref{table:communication}.

\begin{table}[h]
\centering
\caption{Communication Overhead}\label{table:communication}
\begin{tabular}{l|c|c}
\hline\hline
\multicolumn{3}{c}{Authority}\\\hline
 & Send (bits) & Receive (bits) \\\hline
\textsc{Initialize}& 8$\kappa$ & 8$\kappa$ \\
\textsc{Keygen} & $4n\kappa(n-n_{min})$ & $4(n-1)\kappa(n-n_{min})$\\
\textsc{Encrypt} \& \textsc{Decrypt} & 0 & $\abs*{\mathcal{P}}\kappa$ \\\hline\hline
\multicolumn{3}{c}{Per Participant}\\\hline
	& Send (bits) & Receive (bits) \\\hline
\textsc{Initialize} & 8$\kappa$ & 8$\kappa$ \\
\textsc{Keygen} & $4n\kappa(n-n_{min})$ & $4(n-1)\kappa(n-n_{min})$\\
\textsc{Encrypt} \& \textsc{Decrypt} & $\kappa$ & 0 \\\hline\hline
\end{tabular}
\end{table}



Note that we only need $1$ round of communication during each data aggregation, i.e., participants do not need to wait for someone else, but they just send out their ciphertexts when ready. This is not true in most of homomorphic encryption based approaches (\cite{castelluccia2005efficient}\cite{castelluccia2009efficient})



\subsection{Computation Overhead}

To evaluate the computation overhead, we implemented our privacy-preserving arithmetic protocol (\ref{section:design}) in Ubuntu 12.04 using the GMP library (gmplib.org/) based on C in a computer with Intel i3-2365M CPU @ 1.40 GHz $\times 4$, Memory 4GB and SATA Hard Drive 500GB (5400RPM). To exclude the communication overhead from the measurement, we generated all the communication strings (ciphertexts) and conducted all the computation at a local computer. Every algorithm is executed 1000 times to measured the average run time.

To see the influence of the security parameter $\kappa$, we fixed the number of total participants at 10, and measured the run time of every algorithm in the privacy-preserving arithmetic protocol on different $\kappa$ (Fig. \ref{fig:result-a}-\ref{fig:result-d}, ). The run time of multiplicative encryption dominates the one of multiplicative decryption as shown in \ref{fig:result-d}. We can see the \textsc{Encrypt}'s overhead is quite low. Addition needs 2.16 $\mu$s and multiplication needs 1.458 ms when $\kappa=1024$.

Then, to see how the run time grows w.r.t the $n$ (upper bound of the participants in the system), we fixed $\kappa=128$ and measured the run time on different $n$ (Fig. \ref{fig:result-e}-\ref{fig:result-h}). To see the worst-case run time, we let all $n$ participants participate in the sum calculation and product calculation (Fig. \ref{fig:result-g},\ref{fig:result-h}). Clearly, the run time of the \textsc{Keygen} grows quadratically, which is due to the $n-1$ interactions in each $Keygen_i$ for $i=1,\cdots,n$. \textsc{Initialize} and \textsc{Encrypt} are only relevant to the security parameter, while \textsc{Decrypt} grows linearly since it needs to add or multiply all ciphertexts from $n$ participants. The $n$ is small in our setting, but it can be huge since the most computationally intensive operation is the quadratically growing algorithm \textsc{Keygen}, which is a one-time operation.

\begin{figure*}[!t]
  \begin{center}\vspace{-15pt}
    \subfigure[\textsc{Initialize} on various $\kappa$]{\label {fig:result-a}\includegraphics[scale=0.145]{origin/initialize.pdf}}
    \subfigure[\textsc{Keygen} on various $\kappa$]{\label {fig:result-b}\includegraphics[scale=0.145]{origin/keygen.pdf}}
    \subfigure[Additive \textsc{Encrypt} \& \textsc{Decrypt} on various $\kappa$]{\label {fig:result-c}\includegraphics[scale=0.145]{origin/additive.pdf}}
    \subfigure[Multiplicative \textsc{Encrypt} \& \textsc{Decrypt} on various $\kappa$]{\label {fig:result-d}\includegraphics[scale=0.145]{origin/multiplicative.pdf}}
        \subfigure[\textsc{Initialize} on various $n$]{\label {fig:result-e}\includegraphics[scale=0.145]{origin/initialize_n.pdf}}
    \subfigure[\textsc{Keygen} on various $n$]{\label {fig:result-f}\includegraphics[scale=0.145]{origin/keygen_n.pdf}}
    \subfigure[Additive \textsc{Encrypt} \& \textsc{Decrypt} on various $n$]{\label {fig:result-g}\includegraphics[scale=0.145]{origin/additive_n.pdf}}
    \subfigure[Multiplicative \textsc{Encrypt} \& \textsc{Decrypt} on various $n$]{\label {fig:result-h}\includegraphics[scale=0.145]{origin/multiplicative_n.pdf}}
  \end{center}
  \vspace{-11pt}
  \caption{Computation Overhead Measurement}
  \vspace{-15pt}
  \label{fig:result}
\end{figure*}

We further compare the performance of our protocol with MPEP  \cite{jung2013privacypreserving} (Fig. \ref{fig:result2}). It is clear that our scheme is much fater than MPEP in any condition.

\begin{figure}[h]
  \begin{center}
    \subfigure[Sum calculation among $n$ participants]{\label {fig:result2-a}\includegraphics[scale=0.23]{origin/compare_add.pdf}}
    \subfigure[Product calculation among $n$ participants]{\label {fig:result2-b}\includegraphics[scale=0.23]{origin/compare_mul.pdf}}
  \end{center}
  \vspace{-11pt}
  \caption{Comparison with MPEP \cite{jung2013privacypreserving}}
 \label{fig:result2}
\end{figure}

==> problem_v1.tex <==
\section{Provably Secure \ourprotocol}


\subsection{Definitions}


We begin with a precise definition of the provably secure data publishing scheme, followed by formal security definitions. Without the loss of generality, we assume there are $n$ users within the system in total, and each user is represented by an integer ID $\in\{1,\cdots,n\}$.
\begin{definition}
The provably secure data publishing scheme \ourprotocol is a collection of the following four polynomial time algorithms: $(\mathsf{Setup}, \mathsf{KeyGen}, \mathsf{Encode}, \mathsf{Aggregate})$.

$\mathsf{Setup}(1^\kappa)\rightarrow \mathsf{params}$ is a probabilistic setup algorithm that is run by a crypto server to generate system-wide public parameters $\mathsf{params}$ given a security parameter $\kappa$ as input.

$\mathsf{KeyGen}(\mathsf{params})\xrightarrow{dist.}\{\SK_1,\SK_2,\cdots,\SK_n\}$ is a probabilistic and distributed algorithm jointly run by the users. Each user $i$ will secretly receive his own secret key $\SK_i$.

$\mathsf{Encode}(x_i)\rightarrow \mathcal{C}_i$ is a probablistic algorithm run by each user $i$ to encode his private value $x_i$ into a communication string $\mathcal{C}_i$. The output $\mathcal{C}_i$ is published as 


$\mathsf{Aggregate}(\{\mathcal{C}_i\})\rightarrow f(\mathbf{x})=\sum(c_j\prod x_i^{e_{ij}})$
\end{definition}



\subsection{Problem Statements}

Our privacy-preserving data aggregation problem is to let aggregater(s) compute multivariate polynomials (Eq. \ref{equation:polynomial}) among any group of participants $\mathcal{P}\in\{1,\cdots,n\}$  while satisfying aforementioned requirements. 

%To solve it, we present a flexible arithmetic protocol which let any participants  compute their sum and product privately. The protocol as well as its security model is defined in this section.


\subsection{System \& Adversarial Model}

We use an integer value to represent a participant (i.e., ID), and \textit{w.l.o.g} we assume the participants' public IDs are $\{1,\cdots,n\}$ where $n$ is the upper bound of acceptable participants in the system, which can be very large. On the other hand, there is a minimum requirement for each data aggregation, which defines the required minimum number of participants in each transaction, denoted as $n_{min}$.  The powers $\{d_{i,k}\in\zgroup_{p-1}\}$ and coefficients $\{c_{i,k}\in\zgroup_p\}$ of Eq. \ref{equation:polynomial} are public parameters known to anyone, and each participant $i$ has a privately known integer data $x_i\in\zgroup_p$, where $p$ is a large prime number. We assume that the final result $f(\textbf{x}_{\mathcal{P}})$ is positive and bounded by a large prime number $p$.



Two different models are considered: \emph{Authority-Participant Model} and \emph{All-Participants Model}.\smallskip

\textbf{Authority-Participant Model}:
In this model, we have one authority  and ordinary participants.  The authority is the aggregater who wants some aggregate information out of participants' data. We assume the authority is untrustful and curious. That is, he always eavesdrops all the communications and tries to harvest their input data. We also assume participants are curious as well, but they will follow the protocol in general and only part of them will collude with others except the authority such that each collusion group only has up to $n_{min}-2$ participants. In this model, only the authority learns the final aggregate information. 

This model is applicable to a case similar to the data mining application in which users provide individual data and an authority needs some statistics out of it.\smallskip

\textbf{All-Participant Model}:
The second model is consist of ordinary participants only, and they are all assumed to be curious, but follow the protocol in general. Likewise, the size of the collusion group is not greater than $n_{min}-2$. Every participant who participates in the aggregation learns the final aggregation information, but other participants who do not join the aggregation transaction learn nothing from their aggregation. 

This model is applicable to a case similar to the crowd sourcing application in which `crowds' need to share a function of their private data.\medskip


$n_{min}$ is a system-wide parameter  $\geq 2$ in the authority-participant model and $\geq 3$ in the all-participants model. 2 and 3 are lower bounds of $n_{min}$ in two models, which is an inherent requirement of any privacy-preserving multivariate polynomial evaluation (revealing $x_1+x_2$ or $x_1x_2$ while keeping $x_1,x_2$ secret is not possible). Higher $n_{min}$ can be used in applications which requires certain number of participants.



%The objective of the aggregator or the participants is to  compute the polynomial Eq. \ref{equation:polynomial} without knowing any individual $x_i$. 






%\subsection{Additional Assumptions}
%
% 
%We assume that the discrete logarithm problem
%is computationally hard if the involved integers  are large numbers (base, exponent and modulo) except the special case (Section \ref{section:preliminary}) we exploit in our construction. The security of our scheme relies on this assumption similar to other peer cryptographic works (\cite{jung2013privacy}\cite{zhang2013verifiable}\cite{li2013search}). In addition, we also assume that a user authentication was in place to authenticate each participant and their transmission.


%We further assume that there exists a secure pseudorandom function (PRF) which can choose a random element from a group such that this element is computationally indistinguishable to uniform random.
%One example could be the random number generator in Unix system, whose seed is calculated based on the noise created by I/O devices of a computer. This noise is unpredictable if its entropy is high enough (i.e., there are lots actions or movements from I/O devices), and thus the generated random number is considered to be uniform random.

%Dong \emph{et al.} \cite{dong2011secure} investigated verifiable privacy-preserving dot product of two vectors and Zhang \textit{et al.} \cite{zhang2013verifiable} proposed verifiable multi-party computation, both of which can be partially or fully exploited later. Designing privacy preserving data aggregation while providing  verification of the correctness of the provided data is a future work.







 
 

\subsection{Security Model}

%An authority or a participant who joins the data aggregation is the most powerful adversary in this scheme since they have the most information. Denote the probability to correctly infer $v$ as Pr$[v]$, then
%
%\begin{definition}
%An adversary's advantage over participant $i$'s private data is
%\end{definition}
%
%{\footnotesize\vspace{-11pt}
%\begin{displaymath}
%adv_{i}=\text{Pr}[x_i|\mathcal{C},\textsf{Output}]-\text{Pr}[x_i|\textsf{Output}]
%\end{displaymath}\vspace{-14pt}}
%
%\noindent \textit{where $\mathcal{C}$ is all communication strings throughout the scheme and \textsf{Output} is adversary's output of the scheme.}
%
%\begin{definition}
%An adversary's advantage over the final aggregation result is
%\end{definition}
%
%{\footnotesize\vspace{-11pt}
%\begin{displaymath}
%adv_{f}=\text{Pr}[f(\textbf{X}_\mathcal{P)}|\mathcal{C},\textsf{Output}]-\text{Pr}[f(\textbf{X}_\mathcal{P)}|\textsf{Output}]
%\end{displaymath}\vspace{-14pt}}



\noindent \textbf{Start} The challenger creates two virtual participants: $\{1,2\}$. Then, he runs the \textsc{Setup} algorithm and gives the public key to the adversary.

\noindent \textbf{Phase 1}
The adversary creates up to $n_{min}-2$ virtual participants: $\{3,\cdots,n_{min}\}$, where $n_{min}$ is the minimum requirement of the participants number in any transaction. Then, all the virtual participants $\mathcal{P}=\{1,\cdots,n_{min}\}$ jointly run \textsc{Initialize}\footnote{To be secure against $n_{min}$-2 collusion attacks, participant 1,2 are adjacent in the ring formation proposed in \cite{jung2013privacypreserving}} and \textsc{KeyGen} to achieve their master keys and encryption keys.


\noindent \textbf{Challenge}
The adversary randomly chooses $x_3,\cdots,x_{n_{min}}\in\zgroup_p$ for his virtual participants. Then, he tells the challenger whether he wants to compute (sum of $\textbf{x}_\mathcal{P}$ or product of $\textbf{x}_\mathcal{P}$). The challenger randomly picks two values $x_1,x_2\in\zgroup_p$ and encrypt them additively (multiplicatively) and sends the ciphertexts to the adversary.

\noindent \textbf{Guess}
The adversary gives a guess $x'$ of $x_1$.\smallskip

The adversary's advantage $\epsilon$ is defined as Pr$[x'=x_1]$.


\begin{definition}
Our privacy-preserving arithmetic protocol is secure if any probabilistic polynomial time adversary (PPTA) $\adv$'s advantage $\epsilon$ is negligible w.r.t the security parameter in the above game, i.e., $\epsilon<|\frac{1}{f(\kappa)}|$ for any polynomial $f(\cdot)$.
\end{definition}



==> scheme_v1.tex <==
\section{Data Aggregation Among Any-Combination Participants}\label{section:scheme}

\subsection{Authority-Participant Model}

\subsubsection{Initialization} 
At first, the system is set up (i.e., \textsc{setup} algorithm is executed by the authority), and the public key $\PK$ is published. Then, the authority creates a virtual participant with ID $n+1$ ($n$ is the upper bound for the participants number), and all real participants $1,\cdots,n$ as well as virtual participant $n+1$ participate in the one-time key generation including \textsc{Initialize} and \textsc{Keygen}. Real participants as well as virtual participants receive their encryption keys privately.

\subsubsection{Encryption}
Whenever the authority needs to compute an aggregation function (Eq. \ref{equation:polynomial}), he declares the polynomial (the group of real participants $\mathcal{P}$ is implied in the polynomial description), and every (real and virtual) participant sets $\mathcal{P}^*=\mathcal{P}\cup\{n+1\}$. Then, every real participant $i\in\mathcal{P}$ encrypts his private data set $\{c_{ij}x_i^{d_{ij}}\}_{j=1,\cdots,m}$ (denoted as $\{\hat{x}_{ij}\}_{j=1,\cdots,m}$ hereafter) to multiplicative ciphertexts $\{\mathcal{E}^{\times}(\hat{x}_{ij})\}_{j=1,\cdots,m}$ using the algorithm \textsc{Encrypt}($\PK,\SK_i,\mathcal{P}^*,\hat{x}_{ij}$). All ciphertexts are sent to the authority.

\subsubsection{Aggregation}
The authority recovers each single product term $\prod_{i\in\mathcal{P}}\hat{x}_{ij}$ in Eq. \ref{equation:polynomial} by computing the following for all $j=1,\cdots,m$:\vspace{-10pt}


%{\footnotesize\vspace{-4pt}
\begin{displaymath}\begin{split}
&g^{R_{n+1}^{(\abs*{\mathcal{P}^*})}\mathcal{L}_{n+1,\hat{P}^*}(0)}\textsc{Decrypt}(\PK,\{\mathcal{E}^{\times}(\hat{x}_{ij})\}_{i\in\mathcal{P}})\\
=&\prod_{i\in\mathcal{P}}\hat{x}_{ij}\mod p
\end{split}\end{displaymath}\vspace{-4pt}
%\vspace{-8pt}}


\noindent Then, he adds them all to recover the final $f(\textbf{x}_\mathcal{P})$.\smallskip

\noindent \textbf{Special Case}

The aggregater is aware of every product term's value, which leads to the following special case. If there is only one value in a product term (i.e., $\prod_{i\in\mathcal{P}}\hat{x}_{ij}=\hat{x}_{kj}$ for some $k$), the participant $k$'s private value $\hat{x}_{kj}$ is directly revealed to the aggregater. Denote these single-value product terms as $\Sigma=\{\hat{x}_{ij}\}$. In this case, the owners of the values in $\Sigma$ form a new group $\mathcal{P}_{\Sigma}$, and the following is conducted to compute their sum.

\subsubsection{Extra Encryption}
Every participant $i\in\mathcal{P}_\Sigma$ sets $\mathcal{P}^*_\Sigma=\mathcal{P}_\Sigma\cup\{n+1\}$, and encrypts his private data $\hat{x}_{ij}\in\Sigma$ to an additive ciphertext $\mathcal{E}^+(\hat{x}_{ij})$, which is sent to the authority.\smallskip

\subsubsection{Extra Aggregation} 
The authority recovers the sum by computing the following:\vspace{-4pt}

%{\footnotesize\vspace{-6pt}
\begin{displaymath}
R_{n+1}^{(\abs*{\mathcal{P}})}+\textsc{Decrypt}(\PK,\{\mathcal{E}^+(\hat{x}_{ij})\}_{i\in\mathcal{P}_\Sigma})=\sum_{i\in\mathcal{P}_\Sigma}\hat{x}_{ij}\mod p
\end{displaymath}\vspace{-4pt}
%\vspace{-10pt}}

\noindent After which all product terms and the sum are added together, which yields $f(\textbf{x}_\mathcal{P})$.


Although all transmission is open to anyone due to the insecure channels, only the authority learns $f(\textbf{x}_\mathcal{P})$ because others do not know his encryption key $\SK_{n+1}$, and each participant's individual values are not disclosed because their encryption keys are unknown, too.





\subsection{All-Participants Model}

\subsubsection{Initialization} 
At first, the system is set up by any participant, and the public key $\PK$ is published. Then, the participants are engaged in a one-time key generation including \textsc{Initialize} and \textsc{Keygen}, after which all participants retrieve their encryption keys privately.\smallskip

\subsubsection{Encryption}
Whenever a data aggregation is required, every participant $i\in\mathcal{P}$ encrypts his private data set $\{\hat{x}_{ij}\}_{j=1,\cdots,m}$ multiplicatively, and the ciphertexts are broadcast to everyone.\smallskip

\subsubsection{Aggregation}
Every participant $i\in\mathcal{P}$ executes \textsc{Decrypt} to recover each product terms:

{\vspace{-8pt}
\begin{displaymath}
\textsc{Decrypt}(\PK,\{\mathcal{E}^{\times}(\hat{x}_{ij})\}_{i\in\mathcal{P}})=\prod_{i\in\mathcal{P}}\hat{x}_{ij}\mod p
\end{displaymath}\vspace{-6pt}
}

Then, every participant adds them all to compute the $f(\textbf{x}_\mathcal{P})$ locally. Note that the same special case exists as well, and similar extra two phases are needed to calculate $\Sigma$'s sum privately, which is omitted due to space limit.
